mmDrive: mmWave Sensing for Live Monitoring and On-Device Inference of Dangerous Driving

Detecting dangerous driving has been of critical interest for the past few years. However, a practical yet minimally intrusive solution remains challenging as existing technologies heavily rely on visual features or physical proximity. With this motivation, we explore the feasibility of purely using mmWave radars to detect dangerous driving behaviors. We first study characteristics of dangerous driving and find some unique patterns of range-doppler caused by 9 typical dangerous driving actions. We then develop a novel Fused-CNN model to detect dangerous driving instances from regular driving and classify 9 different dangerous driving actions. Through extensive experiments with 5 volunteer drivers in real driving environments, we observe that our system can distinguish dangerous driving actions with an average accuracy of > 95%. We also compare our models with existing state-of-the-art baselines to establish their significance.

==> tex/literature_backup.tex <==
% While solving the problem of monitoring dangerous driving behaviors, the existing literature branches out in multiple directions. Here, we summarize the most notable works in each of these directions.
The existing literature on monitoring dangerous driving behaviors branches out in multiple directions. Here, we summarize the most notable works in each of these directions.
\paragraph*{Orientation and abnormality-based approaches} 
These older approaches~\cite{ersal2010model, dai2010mobile} assess the orientation of the vehicle defined by a set of parameters such as position, velocity, acceleration, etc., and subsequently  exploit them to \textit{indirectly} monitor dangerous driving.  The assumption here is that the abnormality in the driving behavior causes irregular patterns in these parameters, eventually inferring dangerous driving. However, several uncontrollable elements, such as weather, traffic, etc., could also cause irregularity in driving patterns and, therefore, not necessarily signify dangerous driving. Thus, more \textit{direct} monitoring such as vision-based systems have subsequently gained popularity.
% Subsequently, \textit{direct} monitoring of the such as vision-based systems.
% In this direction, the primary objectives are to assess the orientation~\cite{ersal2010model, dai2010mobile} of the vehicle defined by a set of parameters such as position, velocity, acceleration, etc. In this \textit{indirect} way of monitoring, researchers have exploited abnormality in the parameters mentioned above. The assumption is that the abnormality in the driving behavior will cause irregular patterns in these parameters, eventually inferring an inattentive and dangerous driving scenario. However, it is worth noting that several uncontrollable elements, such as weather conditions, traffic conditions, and the like, could also cause irregularity in driving patterns and, therefore, not necessarily signify a dangerous driving pattern. Motivated by this, researchers, therefore, opted for vision-based ideas towards \textit{direct} monitoring of the driver.

\paragraph*{Vision-based approaches} 
Vision-based approaches~\cite{cyganek2014hybrid, borghi2017poseidon} leverage computer vision on RGB camera~\cite{dua2020dgaze}, thermal imaging~\cite{kajiwara2021driver}, and Infrared (IR) camera~\cite{yan2011robust} data, to detect abnormal driving activities by directly focusing on the driver. The captured images within the environment are processed to determine movements including facial features such as eye movements, talking, and yawning, as well as movements of other body parts~\cite{hoang2016multiple} such as head movements, hand movements, etc. These activities, in turn, signify patterns of inattentive or dangerous driving behaviors. However, such vision-based approaches potentially incur invasion of privacy~\cite{zhang2016privacy}, limiting their adoption as a pervasive practical solution.
% Vision-based approaches~\cite{cyganek2014hybrid, borghi2017poseidon} leverage computer vision to detect relevant abnormal driving activities by directly focusing on the driver. Apart from an RGB camera~\cite{dua2020dgaze}, thermal imaging~\cite{kajiwara2021driver} and Infrared (IR) cameras~\cite{yan2011robust} were also used for this purpose. The captured images within the environment are processed to determine various relevant activities of a driver. These movements include facial features such as eye movements, facial expressions, talking, and yawning, as well as movements of other body parts~\cite{hoang2016multiple} such as head movements, hand movements, and the like. These activities, in turn, signify patterns of inattentive or dangerous driving behaviors. However, with the capturing of image data, the vision-based approach incurs invasion of privacy~\cite{zhang2016privacy}, thereby making it difficult to be adopted as a pervasive practical solution.
\paragraph*{Wearable-based approaches} Considering the pervasiveness and effectiveness of wearable devices, researchers have leveraged them to sense body kinematics and other body-specific signatures. Patterns in IMU (Inertial Measurement Unit) information, EEG (ElectroEncephaloGram)~\cite{cisotto2018joint} signals, heart rate, etc., bear various activity-specific signatures, and thus are used to eventually assess abnormal and dangerous driving behaviors. However, there also exist critical challenges with the leveraging of wearables. Firstly, the signatures collected from one age group do not always fit well with the signatures of a different age group, making it difficult to make such a system generic. Additionally, wearables such as sensors of EEG fitted on the head/body have some invasive footprints and interfere with individuals' day-to-day movements. Therefore, using them may not be a practical solution for continuous monitoring under every possible circumstance.


% In the current times of IoT (Internet of Things), the tendency to keep every object individual \textit{connected} has resulted in many wearable devices. Considering their pervasiveness and effectiveness, researchers have therefore leveraged them to sense different factors such as body kinematics and other body-specific signatures. In this direction, various sensors to capture IMU (Inertial Measurement Unit) information, EEG (ElectroEncephaloGram)~\cite{cisotto2018joint} signals, heart rate, etc., were explored. The captured patterns, in turn, bear various activity-specific signatures, which are then referred to eventually assess abnormal and dangerous driving behaviors. However, there also exist critical challenges with the leveraging of wearables. Firstly, the signatures collected from one age group do not always fit well with the signatures of a different age group, making it difficult to make such a system generic. Additionally, wearables such as sensors of EEG fitted on the head/body have some invasive footprints and interfere with individuals' day-to-day movements. Therefore, using them may not be a practical solution for continuous monitoring under every possible circumstance.
\paragraph*{Acoustics-based approaches} Researchers have also explored acoustics for studying distracted and dangerous driving scenarios. It can be seen from the literature that within the in-car environment, Doppler shifts from acoustic signals~\cite{xu2017er, xie2019d} as well as FMCW chirps~\cite{jiang2021driversonar} could be effective to detect abnormal body movements of the driver. The captured patterns are then analyzed to predict improper driving scenarios. However, one cannot ignore the fact that environmental noise has a significant influence~\cite{bai2020acoustic} over acoustic-based sensing. Other factors, such as the influence of location, Orientation, and even privacy issues, could also be of concern with acoustic sensing. Even with arguably pervasive devices such as smartphones when used for acoustic sensing, it is worth noting that different devices have different sensitivity patterns~\cite{hromadova2022frequency} for audio signals.

==> tex/prelims_back.tex <==
\section{Background and
Observations}
In this section first we introduce the common dangerous driving actions. Then we present the principle of FMCW based mmWave radar in sensing these driving actions. Finally we explore the feasibility of mmWave sensing in detection of dangerous driving actions. 
\subsection{Dangerous driving actions}\label{sec:dda}
Drivers encounter various road accidents because of being in inattentive state while driving. These inattentive states primarily can be categorized into two groups: actions related to drowsy driving and actions related to distracted driving. We briefly discuss each of these dangerous driving actions below.     
\subsubsection{Actions related to Drowsy Driving} This group of actions typically involves dangerous driving behaviors caused due to drowsiness.
\begin{itemize}[leftmargin=*]
    \item \textbf{Nodding} Since it is difficult for a driver to see nearby road conditions when resting their head on the headrest, as shown in Fig.~\ref{}, a driver's head always has a tiny gap with the headrest when driving regularly. But when a driver is feeling drowsy, he/she typically make a fast periodic bowing motion of the head in front and back direction while nodding, as seen in Fig.~\ref{}.
    \item \textbf{Yawning} A common action when drivers are fatigued is yawning. The two acts that make up a yawn include opening the mouth widely for inspiration, lifting the head due to the reactive force of expiration, and finally lowering the head to its normal position, as shown in Fig.~\ref{}.
    \item \textbf{Anomaly in steering} A typical driver often turns the steering wheel smoothly and softly, even on straight highways. The capacity to control a vehicle, namely the frequency of steering wheel adjustments, gradually declines as drowsiness progresses. Vehicles move laterally for a longer distance if the driver cannot adjust the driving orientation in time. When the driver becomes abruptly aware of the situation, he or she quickly adjusts the steering wheel to change the vehicle's direction, as seen in Fig.~\ref{}.
\end{itemize}
\subsubsection{Actions related to distracted driving} Distracted driving actions typically include eating or drinking, turning back, picking drops, using a mobile phone, speaking to someone, etc.
\begin{itemize}[leftmargin=*]
    \item \textbf{Drinking or Eating} As seen in Fig.~\ref{}, eating or drinking while driving might cause a minor forward tilt followed by oscillations back and forth. Additionally, one hand is momentarily taken off the wheel to deliver food to the mouth.
    \item \textbf{Turning back} Drivers may turn around to check on baggage or goods left in the backseat or care for their children in the backseat as shown in Fig.~\ref{}.
    \item \textbf{Picking drops} As shown in Fig.~\ref{}, driver may intend to pick dropped items from the car floor while driving.
    \item \textbf{Fetching forward} Driver may intend to lean forward to fetch something from the car dashboard while driving, as shown in Fig.~\ref{}.
    \item \textbf{Using Mobile Phone} During distracted driving state driver may use his/her mobile phone while driving, keeping one hand on steering and the other hand close to his mouth.  
    \item \textbf{Talking to person in left} The driver may intend to speak with the passenger sitting in the adjacent seat, as shown in Fig.~\ref{}.
\end{itemize}
Based on the actions mentioned above, we can conclude that each unsafe driving behavior is not transitory but lasts for a while. Additionally, we notice that, whether on purpose or accidentally, the head position and the motion pattern of the steering hand during dangerous driving acts differ from those in normal driving conditions. Therefore, using the real-time head position change and steering hand motion pattern is reasonable to spot dangerous driving behaviors. We use FMCW mmWave Radar to capture the patterns of driver actions. 
\subsection{Principle of mmWave Sensing}
We first introduce the essential factors involved with an mmWave radar which are relevant to capture the aforementioned dangerous driving actions.
\begin{figure}
    \centering
    \subfigure[]{
    \includegraphics[width=0.21\textwidth]{figures/driver_sitting.drawio.pdf}
    \label{fig:radar_placement}}
    \subfigure[]{
    \includegraphics[width=0.24\textwidth]{figures/fmcw_radar_drawio.pdf}
    \label{fig:fmcw_working}}
    \caption{ Working principle of an FMCW Radar - (a) Radar Placement (b) chirp frequency vs time.} 
        \label{fig:mmwavefunction}
  \end{figure}
  
The primary working principle of an mmWave radar involves the transmission of short wavelength ($1$-$10$ mm) and wide frequency band ($4$GHz) electromagnetic waves. Because of this wide frequency band ($4$GHz), it has a high range resolution ($\approx4$ cm) and is suitable for distinguishing different actions of the human body.

Frequency Modulated Continuous Wave (FMCW) is the most commonly used modulation scheme for automotive mmWave radars. FMCW radar system mainly includes a transceiver antenna, RF front-end, modulation signal, a signal processing module, etc. The radar receives the reflection from objects or user present within the Line-of-sight (LOS)  to estimate the \textit{range, velocity, and angle}. 

FMCW radar uses a linear \textit{`chirp'} or swept frequency transmission. When receiving the signal reflected by the driver or other objects in the field-of-view (FoV), the radar performs a dechirp operation by mixing the transmitted signal with the reflected signal, producing an Intermediate Frequency (IF) signal. Now to determine the position and body movements of the driver signal processing techniques are carried out on this IF signal.  
\subsubsection{Determining position of the driver}\label{subsec:range}
FMCW radar generates continuous waves in the form of periodic signals (\textit{`chirp'}) where the frequency increases linearly with time. There is a certain frequency difference between the transmitted signal and the signal reflected by the target. The distance information between the target and the radar can be obtained by measuring this frequency difference~\cite{iovescu2020fundamentals}.

As shown in Fig.~\ref{fig:fmcw_working}, suppose we have a transmitted chirp (TX chirp) with transmission time $T_C$. Due to presence of the driver at a distance of $d$ from the radar, we have a received chirp (RX chirp) after a round-trip-time of $\tau$. The IF signal generated by mixing the TX and RX chirp has a beat frequency, say $f_b$. The slope ($S$) of this FMCW chirp can be represented as,
\begin{equation}
    S = \frac{B}{T_C} = \frac{f_b}{\tau}
\end{equation}
Also, the round-trip-time $\tau$ can be derived as,
\begin{equation}
    \tau = \frac{2d}{c}
\end{equation}
where $d$ is the distance of the detected driver or other reflector object and $c$ is the speed of light. 
Thus, the distance of the driver can be given as,
\begin{equation}\label{eq:range}
    d = \frac{c}{2} . \frac{T_C}{B} . f_b
\end{equation}
To sum up, the detection range of the FMCW radar is determined by Equation \ref{eq:range}, and the key parameter is the frequency difference ($f_b$) between TX and RX chirp. Now to determine this beat frequency a Fast Fourier Transform (FFT) is conducted on the IF signal ($f_b$). This FFT also called as range-FFT produces frequency peaks at locations where the driver or other reflectors are present. And based on equation~\ref{eq:range}, the corresponding range is calculated. This information is captured in the form of a 1D array called as \textit{range profile} representing received power at different range bins.
\subsubsection{Determining body movements of the driver}
In order to measure body movements or velocity, an FMCW radar transmits $N$ number of chirps separated by a transmission time of $T_C$. On applying range-FFT (as discussed in Sec.~\ref{subsec:range}), the objects present at different locations are captured. If the driver is having body movements, then the range-FFT corresponding to each chirp will have peaks in the same location but with a different phase. If the driver is moving with a speed of $v$, the measured phase difference between two successive RX chirps corresponding to a motion of $v\times T_C$ can be given as,
\begin{equation}
    \Delta \phi = \frac{4\pi (v \times T_C)}{\lambda}
\end{equation}
A second FFT, called \textit{Doppler-FFT}, is performed on these N phasors to determine the movement of the driver. Thus by including both the range information and the doppler information, we can capture the position of the driver as well as their body movement. This information is captured in the form of a 2D matrix called \textit{range-doppler} heatmap. Also, this doppler information at different range bins help in calculating the \textit{noise profile}, which is in the same format as \textit{range profile} but the profile is at the maximum Doppler bin (maximum body movements). In general for normal driving scene, there would be lesser body movements or lesser clutter at maximum speed so the range profile at such speed represents the receiver noise floor.

Next, we will explore variation of \textit{range-doppler}, \textit{range profile} and \textit{noise profile} across different driver's behavior.
\subsection{Analyzing Patterns of Dangerous Driving Actions}
To analyze different dangerous driving action patterns we place the mmWave radar in the car dashboard in front of the driver as shown in Fig.~\ref{fig:radar_placement}. With the given placement we explore variation in the \textit{range-doppler}, \textit{range profile} and \textit{noise profile} across different driving behaviors. As discussed in Section~\ref{sec:dda} each of the dangerous driving actions has unique body movement patterns and activity time. For example, while picking drop from car floor driver bends his/her body downwards and picks up the item and returns back to normal gesture. For Fetching forward driver brings his/her body forward towards the dashboard and after fetching the item returns back to usual position. These activities produce unique patterns in the \textit{range-doppler} heatmap as shown in Fig.~\ref{fig:raw_range_doppler}. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/range_doppler.pdf}
    \caption{Variation of Range-doppler heatmap across different dangerous driving actions}
    \label{fig:raw_range_doppler}
\end{figure}

\subsubsection{Variation in the range-doppler heatmap}
The \textit{range-doppler} information is in the form of a 2D image where it's abscissa is the range, the ordinate is the Doppler speed, and the value contained is the power value of velocity across different range and doppler bins. Typical distance between the driver and mmWave sensor is around $0.6$ to $0.8$ meters, which represents range bins from 6 to 16. Thus we observe a higher power value in this range as seen in Fig.~\ref{fig:raw_range_doppler}. For body movements such as fetching forward, picking drops, nodding, turning back, etc., driver moves his/her body in a particular direction, stays in that orientation for a few seconds and then returns back to normal position. For these types of actions we observe when the driver starts the activity the doppler shifts up in positive direction (or negative depending upon the direction of movement). When driver finally returns to normal state the doppler shifts down (or up depending on direction of movement) and finally comes back to zero doppler line when the activity ends. Thus we observe a circular pattern in the range-doppler heatmap for the given activities  as shown in Fig.~\ref{fig:raw_range_doppler}. For anomaly in steering driver abruptly moves his steering resulting in sudden change in range-doppler heatmap across different range bins.           
For activities such as yawning, drinking or using mobile phone while driving, driver usually makes less body movements and thus the variation in the range-doppler is less significant for these activities (see Fig.~\ref{fig:raw_range_doppler}). 
\subsubsection{Variation in range-doppler, range profile, noise profile across different user}
Now to understand these variation in more detail in Fig.~\ref{fig:violin_variation} we show distribution of mean of the  range-doppler, range profile, noise profile for different driving actions for two different drivers. As seen in Fig.~\ref{fig:doppler_violin} and Fig.~\ref{fig:noise_violin}, yawning, using phone, talking to the person in left (adjacent seat) or drinking shows lesser variation as the distribution is more dense in the  interquartile range. However for the rest of the driving actions we observe the distribution is less dense towards the median representing macro body movements of the driver. On the other hand Fig.~\ref{fig:range_violin} shows distribution of range profile across different driving actions. Here the variation is less significant across activities, however the location of the medians of range profile for the two users have a significant gap due to difference in driver's height or seat adjustment by the driver. 
\begin{figure}
    \centering
    \subfigure[]{
    \includegraphics[width=0.465\textwidth]{figures/violin_doppler_actions.pdf}
            \label{fig:doppler_violin}}
    \subfigure[]{
    \includegraphics[width=0.465\textwidth]{figures/violin_noise_actions.pdf}
            \label{fig:noise_violin}}
    \subfigure[]{
    \includegraphics[width=0.465\textwidth]{figures/violin_range_actions.pdf}
            \label{fig:range_violin}}
    \caption{Variation in the mean of (a) range-doppler, (b) noise profiles and (c) range profiles across different driving actions for two users}
    \label{fig:violin_variation}
\end{figure}
\subsubsection{Variation in the driving actions over time}\label{sec:obs}
To observe the impact of road bumps in the mmWave features we use a IMU sensor. During road bumps the z-axis of the IMU's accelerometer shows a peak. We plot mean of range-doppler, noise profile and the mean of the IMU data for each second over a time duration of 3 minutes in Fig.~\ref{fig:mean_variation}. As seen in Fig.~\ref{fig:mean_variation} each activities has their own time span and mean value. For example yawning takes place for a smaller time duration and the mean value of range-doppler is also low (almost equal to the mean of normal driving). Driver uses his phone for a longer duration and it is also similar to normal driving behavior except certain peaks where the driver is making major body movements for picking up the phone or moving his hand from the steering. On the other hand Anomaly in steering takes place for a longer duration and it has significant variation in the mean value when compared to normal driving. Thus Fig.~\ref{fig:mean_variation} establishes the fact that each of these driving behaviors has it's own signature in the range-doppler or noise profile and also has it's own completion time. On the other hand in the IMU data there is no variation while the driver is performing these activities. However when there is a road bump at around 170s, the IMU data shows a peak. This peak is also observed in the mean of the range-doppler and noise profile data. Thus overall this observation establishes the fact that each of the driving behaviors have there own spatial as well as temporal variation. And road bumps can directly impact the mmWave features. So for classifying the driving behaviors we need to consider both spatial and temporal variations in the feature space as well as instances where road bumps occur.
\begin{figure}
    \centering
     \includegraphics[width=0.5\textwidth]{figures/bump2.eps}
    \caption{Variation in the IMU data, mean range-doppler and noise profile over time}
    \label{fig:mean_variation}
\end{figure}
\subsubsection{Distribution of driving behaviors in a 2D feature space} Although only observing the mean of range-doppler, range profile and noise profile provides a rough estimation of the feasibility of classification of driving behaviors. The range-doppler heatmap is in the form of a 2D matrix with size of $16\times64$ representing $64$ range bins and $16$ doppler bins. One the other hand  range profile and noise profile is in the form of a 1D array of size $64$, representing $64$ range bins. Thus the total size of the feature space is $(16\times 64) + (64\times 2) = 1152$.  To visualize how each of the dangerous driving actions are separated from the normal driving behavior we lower down the higher dimension ($1152$) feature space to a 2D feature space using T-distributed neighbor embedding (t-SNE) based dimensionality reduction technique. As shown in Fig.~\ref{fig:tsne_pca50_features} we observe dangerous driving actions are separable from the normal driving behavior to some extent. Still there exists some overlap in the features for activities such as normal driving and using phone, normal driving and talking to the person left (in the adjacent seat). Also in real driving due to road bumpings or sudden body movements of the driver (not listed in the dangerous driving actions) can also lead to variation in the range-doppler or noise profile. This can also lead to the overlap in the features between normal driving and dangerous driving actions.

Based on the observations the major takeaways are
\begin{itemize}
    \item Range-doppler, noise profile and range profile shows unique patterns across different driving actions as well as across different drivers.
    \item Each of the driving actions has their unique signature in the time of completion.
    \item Features of dangerous driving actions having micro body movements involved lie very close to normal driving behavior.
    \item In real driving road bumps can also lead to variation in the feature space and thus this can also lead to mis-classification if not properly handled.
\end{itemize}
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/tsne.pdf}
    \caption{Distributions of Normal Driving with other dangerous driving actions in 2-dimensional feature space}
    \label{fig:tsne_pca50_features}
\end{figure}
Finally based on the takeaways we next discuss the design of \ourmethod for classifying different driving behaviors.
